Domain Adaptation in Dialogue Systems using Transfer and Meta-Learning

Current generative-based dialogue systems are data-hungry and fail to adapt to new unseen domains when only a small amount of target data is available. Additionally, in real-world applications, most domains are underrepresented, so there is a need to create a system capable of generalizing to these domains using minimal data. In this paper, we propose a method that adapts to unseen domains by combining both transfer and meta-learning (DATML). DATML improves the previous state-of-the-art dialogue model, DiKTNet, by introducing a different learning technique: meta-learning. We use Reptile, a first-order optimization-based meta-learning algorithm as our improved training method. We evaluated our model on the MultiWOZ dataset and outperformed DiKTNet in both BLEU and Entity F1 scores when the same amount of data is available.

==> acronyms.tex <==
% #############################################################################
% This is the ACRONYMS Definition
% !TEX root = ../main.tex
% #############################################################################

\begin{acronym}[H.264/SVC]
	\acro{zsdg}[ZSDG]{Zero-Shot Dialog Generation}
	\acro{fsdg}[FSDG]{Few-Shot Dialogue Generation}
    \acro{diktnet}[DiKTNet]{Dialogue Knowledge Transfer Network}
    \acro{daml}[DAML]{Domain Adaptive Dialogue Generation via Meta Learning}
    \acro{vae}[VAE]{Variational Auto-Encoder}
    \acro{di-vae}[DI-VAE]{Discrete Information Variational Auto-Encoder}
    \acro{laed}[LAED]{Latent Action Encoder-Decoder}
    \acro{di-vst}[DI-VST]{Discrete Information Variational Skip-Thought}
    \acro{hred}[HRED]{Hierarchical Recurrent Encoder-Decoder}
    \acro{seq2seq}[SEQ2SEQ]{Sequence-to-Sequence}
    \acro{rnn}[RNN]{Recurrent Neural Network}
    \acro{cnnet}[CNN]{Convolutional Neural Network}
    \acro{lstm}[LSTM]{Long-Short Term Memory Unit}
    \acro{gru}[GRU]{Gated Recurrent Unit}
    \acro{maml}[MAML]{Model-Agnostic Metal-Learning}
    \acro{kb}[KB]{Knowledge-Base}
    \acro{datml}[DATML]{Domain Adaptation using Transfer Meta-Learning}
    \acro{sos}[SOS]{Start-of-Sequence}
    \acro{eos}[EOS]{End-of-Sequence}
    \acro{nlu}[NLU]{Natural Language Understanding}
    \acro{nlg}[NLG]{Natural Language Generation}
    \acro{dm}[DM]{Dialogue Manager}
    \acro{bleu}[BLEU]{Bilingual Evaluation Understudy}
    \acro{rouge}[ROUGUE]{Recall-Oriented Understudy for Gisting Evaluation }
    \acro{meteor}[METEOR]{Metric for Evaluation of Translation with Explicit ORdering}
\end{acronym}
